Detecting Cohesive and 2-mode Communities in Directed and Undirected Networks

Networks are a general language for representing relational information among objects. An effective way to model, reason about, and summarize networks, is to discover sets of nodes with common connectivity patterns. Such sets are commonly referred to as network communities. Research on network community detection has predominantly focused on identifying communities of densely connected nodes in undirected networks. In this paper we develop a novel overlapping community detection method that scales to networks of millions of nodes and edges and advances research along two dimensions: the connectivity structure of communities, and the use of edge directedness for community detection. First, we extend traditional definitions of network communities by building on the observation that nodes can be densely interlinked in two different ways: In cohesive communities nodes link to each other, while in 2-mode communities nodes link in a bipartite fashion, where links predominate between the two partitions rather than inside them. Our method successfully detects both 2-mode as well as cohesive communities, that may also overlap or be hierarchically nested. Second, while most existing community detection methods treat directed edges as though they were undirected, our method accounts for edge directions and is able to identify novel and meaningful community structures in both directed and undirected networks, using data from social, biological, and ecological domains.

==> 020related.tex <==
% !TEX root = paper-directedagm.tex
Community detection is a vast and well-studied problem that has been approached from many angles \cite{fortunato09community}, and what is a `good' algorithm depends on the specific properties of the network and the types of communities one wishes to detect \cite{fortunato09community}. For example, one may wish to detect communities that are disjoint \cite{karypis98metis}, overlapping \cite{jaewon12agmfit,Ahn10LinkCommunitiesNature,palla05_OveralpNature,demon}, or hierarchically nested \cite{jaewon11comscore}, and different algorithms have been proposed for each case.

% Discussion about overlaps: necessary?
%Classical algorithms for community detection assume that communities are disjoint \cite{Schaeffer07_survey}, though others have modeled hierarchically nested communities \cite{ravasz03_hierarchical}, and communities that partially overlap \cite{Gregory10LabelOverlap,lancichinetti09ovlpbenchmark,Lancichinetti09overlapping,jaewon12agmfit}.

\hide{
Traditionally, communities have been thought of as sets of nodes that are densely interconnected \cite{fortunato09community,palla05_OveralpNature}. However, other notions of what defines a `community' can be found even in early works on the subject \cite{burt78}. There, the authors suggest that communities may be based on \emph{structural equivalence}: nodes with similar connectivity patterns may be considered a community even if they do not connect to each other. A classic example of such communities can be found in \cite{KRRT99_trawling}---there, the authors note that a collection of web pages may be `related' even if they do not link to each other---for example the homepages of various phone-companies are not connected precisely \emph{because} they are competitors.
%TODO: I'm not sure if it's necessary to point out the `flaws' of this paper. It's a seminal paper, so you probably won't get called out for being too similar to it, and maybe it doesn't look so good to sound critical of it.
%JAEWON: Some reviewers said that it is a prior work which decreases our novelty...
When finding communities, \cite{KRRT99_trawling} searches for {\em hard} structural equivalence, which means that the members of a detected community are connected to the same set of other nodes without an {\em any} exception.
However, our work assumes {\em soft} structural equivalence as it is based on a probabilistic framework, which allows us to find communities with different strength of structural equivalence.

%TODO: find the right place to put this
% \jure{move this paragraph later since it is about related work.}
Approaches based on block modeling~\cite{airoldi07blockmodel,Holland83BlockModel} are in principle capable of detecting cohesive as well as 2-mode communities.
% as they model the interactions across and within blocks of nodes.
However, there are two important differences with our work: First, our method scales to networks with millions of nodes, while block modeling approaches typically handle only a few hundred. Second, our method allows for cohesive as well as 2-mode communities to overlap and hierarchically nest inside each other.
%TODO: the above is an example of the type of language we were criticised for

%The notion that not all meaningful network subgroups are based on cohesion is discussed in \cite{burt78}. There, a discussion is given on the aparently competing notions of network communities, namely communities based on cohesive connections, and communities based on common structural properties, or `roles'. They attempt to reconcile the two notions by noticing that indeed, nodes in cohesive communities \emph{do} exhibit structural equivalence, and thus the latter notion is more expressive.

% In the case of web graphs, it was noted in \cite{KRRT99_trawling} that webpages might be considered `related' even if they do not link to each other, for example the homepages of various phone-companies are not connected precisely because they are competitors.

Others have made the observation that traditional definitions of communities in undirected networks may not hold for directed networks \cite{Newman08DirectedCommunity}.
%and that traditional algorithms for undirected networks may fail if na\"ively applied.
In \cite{Newman08DirectedCommunity}, the authors show how traditional definitions of modularity should be adapted to make use of directedness information.
%In \cite{lancichinetti09ovlpbenchmark} They give examples of communities in directed networks based on the concept of flow: two groups may be considered communities if information flows between them, even if they do not communicate internally.
%They also mention that traditional algorithms designed for undirected networks are unlikely to successfully detect such communities.

Recent works on role discovery try to augment traditional node features with features derived from each node's neighbors, i.e., their ego network \cite{Henderson12RolX}. As stated in \cite{Henderson12RolX}, `roles' are complimentary to communities, in that roles are concerned with grouping nodes with similar behavior, rather than grouping nodes based on their connectedness. %In particular, their work differs from ours in that they consider statistics of the neighbors of each node, but not the identity of those neighbors \emph{per se}.
%%Jaewon
% Role is different from communities. Role considers what are your neighbors (\ie, statistics of the neighbors) whereas communities are about ``who'' are your neighbors.
}

We differentiate our approach from methods that explicitly consider community detection in bipartite or heterogeneous networks. For example, one may construct a bipartite graph between \emph{users} and \emph{features}, where an edge between the two groups indicates some property of a user;
% each edge $(u,f)$ indicates that the user $u$ has a feature $f$, even though there are no connections between users or features \cite{barber07}.
the goal is then to discover sets of users whose features are similar.
% for example to discover users who should have similar access permisions \cite{mlsp}.
Although such works offer valuable insights, they differ from ours in that we make no assumption that the networks we study are bipartite or heterogeneous.

%TODO: Tried to rewrite this to *mention* the differences, rather than focusing on the differences per se.
%JAEWON: Thanks!
\model is related to recently developed affiliation graph models~\cite{morup11infinite,jaewon13agmfast,jaewon12agmfit}.
Due to their mathematical elegance and their ability to generate realistic community overlaps~\cite{jaewon13agmtist}, we adopt a similar generative process for \model.
However, a crucial difference is that \model assumes {\em directed} affiliations.
As stated in Fig.~\ref{fig:example}, directed affiliations allow us to model both 2-mode communities and cohesive communities, in both directed and undirected networks.
%TODO: Maybe leave experimental findings out of the related work section? Especially now that this section appears *after* the experimental section.
%JAEWON: Okay. Let's remove it
%Our experiments show that this difference leads to better accuracy in finding the communities in real world networks (Sec.~\ref{sec:experiments}).


% \note{Jure: cut the following paragraph}
% We also differentiate our work from \emph{clustering} algorithms, such as $k$-means and hierarchical clustering \cite{hierarchical,mackay}. Such methods generally group nodes with similar features, and may therefore also be used to facilitate role discovery. However, such `roles' are quite different than what we attempt to model, and without network information it it difficult to distinguish a meaningless feature (such as `hair color') from a meaningful one (such as `celebrity'). Indeed, in Section \ref{sec:?} we show that such methods are not effective in recovering communities in directed networks, even when node features are available.


